Interprocedural Type Specialization of JavaScript Programs Without Type Analysis

Dynamically typed programming languages such as Python and JavaScript defer type checking to run time. VM implementations can improve performance by eliminating redundant dynamic type checks. However, type inference analyses are often costly and involve tradeoffs between compilation time and resulting precision. This has lead to the creation of increasingly complex multi-tiered VM architectures. Lazy basic block versioning is a simple JIT compilation technique which effectively removes redundant type checks from critical code paths. This novel approach lazily generates type-specialized versions of basic blocks on-the-fly while propagating context-dependent type information. This approach does not require the use of costly program analyses, is not restricted by the precision limitations of traditional type analyses. This paper extends lazy basic block versioning to propagate type information interprocedurally, across function call boundaries. Our implementation in a JavaScript JIT compiler shows that across 26 benchmarks, interprocedural basic block versioning eliminates more type tag tests on average than what is achievable with static type analysis without resorting to code transformations. On average, 94.3% of type tag tests are eliminated, yielding speedups of up to 56%. We also show that our implementation is able to outperform Truffle/JS on several benchmarks, both in terms of execution time and compilation time.

==> stats/againsttr_decr_exec_time_only.tex <==
-49

==> stats/againsttr_decr_exec_time_only_1d.tex <==
-49.1

==> stats/againsttr_decr_total_time.tex <==
-144

==> stats/againsttr_decr_total_time_1d.tex <==
-144.3

==> stats/againsttr_incr_exec_time_only.tex <==
49

==> stats/againsttr_incr_exec_time_only_1d.tex <==
49.1

==> stats/againsttr_incr_total_time.tex <==
144

==> stats/againsttr_incr_total_time_1d.tex <==
144.3

==> stats/againsttr_max_decr_exec_time_only.tex <==
72

==> stats/againsttr_max_decr_exec_time_only_1d.tex <==
72.2

==> stats/againsttr_max_decr_total_time.tex <==
34

==> stats/againsttr_max_decr_total_time_1d.tex <==
33.9

==> stats/againsttr_max_exec_time_only.tex <==
2657

==> stats/againsttr_max_exec_time_only_1d.tex <==
2657.5

==> stats/againsttr_max_incr_exec_time_only.tex <==
2557

==> stats/againsttr_max_incr_exec_time_only_1d.tex <==
2557.5

==> stats/againsttr_max_incr_total_time.tex <==
1399

==> stats/againsttr_max_incr_total_time_1d.tex <==
1398.7

==> stats/againsttr_max_total_time.tex <==
1499

==> stats/againsttr_max_total_time_1d.tex <==
1498.7

==> stats/againsttr_mean_exec_time_only.tex <==
149

==> stats/againsttr_mean_exec_time_only_1d.tex <==
149.1

==> stats/againsttr_mean_total_time.tex <==
244

==> stats/againsttr_mean_total_time_1d.tex <==
244.3

==> stats/againsttr_min_exec_time_only.tex <==
28

==> stats/againsttr_min_exec_time_only_1d.tex <==
27.8

==> stats/againsttr_min_total_time.tex <==
66

==> stats/againsttr_min_total_time_1d.tex <==
66.1

==> stats/againsttr_num_above_exec_time_only.tex <==
13

==> stats/againsttr_num_above_exec_time_only_1d.tex <==
13.0

==> stats/againsttr_num_above_total_time.tex <==
23

==> stats/againsttr_num_above_total_time_1d.tex <==
23.0

==> stats/againsttr_num_below_exec_time_only.tex <==
12

==> stats/againsttr_num_below_exec_time_only_1d.tex <==
12.0

==> stats/againsttr_num_below_total_time.tex <==
3

==> stats/againsttr_num_below_total_time_1d.tex <==
3.0

==> stats/againstv8_decr_v8_baseline.tex <==
-153

==> stats/againstv8_decr_v8_baseline_1d.tex <==
-153.2

==> stats/againstv8_decr_v8_full.tex <==
58

==> stats/againstv8_decr_v8_full_1d.tex <==
58.0

==> stats/againstv8_decr_v8_no_inlining.tex <==
40

==> stats/againstv8_decr_v8_no_inlining_1d.tex <==
39.8

==> stats/againstv8_incr_v8_baseline.tex <==
153

==> stats/againstv8_incr_v8_baseline_1d.tex <==
153.2

==> stats/againstv8_incr_v8_full.tex <==
-58

==> stats/againstv8_incr_v8_full_1d.tex <==
-58.0

==> stats/againstv8_incr_v8_no_inlining.tex <==
-40

==> stats/againstv8_incr_v8_no_inlining_1d.tex <==
-39.8

==> stats/againstv8_max_decr_v8_baseline.tex <==
33

==> stats/againstv8_max_decr_v8_baseline_1d.tex <==
32.9

==> stats/againstv8_max_decr_v8_full.tex <==
90

==> stats/againstv8_max_decr_v8_full_1d.tex <==
90.0

==> stats/againstv8_max_decr_v8_no_inlining.tex <==
76

==> stats/againstv8_max_decr_v8_no_inlining_1d.tex <==
76.4

==> stats/againstv8_max_incr_v8_baseline.tex <==
604

==> stats/againstv8_max_incr_v8_baseline_1d.tex <==
604.5

==> stats/againstv8_max_incr_v8_full.tex <==
74

==> stats/againstv8_max_incr_v8_full_1d.tex <==
74.3

==> stats/againstv8_max_incr_v8_no_inlining.tex <==
74

==> stats/againstv8_max_incr_v8_no_inlining_1d.tex <==
74.4

==> stats/againstv8_max_v8_baseline.tex <==
704

==> stats/againstv8_max_v8_baseline_1d.tex <==
704.5

==> stats/againstv8_max_v8_full.tex <==
174

==> stats/againstv8_max_v8_full_1d.tex <==
174.3

==> stats/againstv8_max_v8_no_inlining.tex <==
174

==> stats/againstv8_max_v8_no_inlining_1d.tex <==
174.4

==> stats/againstv8_mean_v8_baseline.tex <==
253

==> stats/againstv8_mean_v8_baseline_1d.tex <==
253.2

==> stats/againstv8_mean_v8_full.tex <==
42

==> stats/againstv8_mean_v8_full_1d.tex <==
42.0

==> stats/againstv8_mean_v8_no_inlining.tex <==
60

==> stats/againstv8_mean_v8_no_inlining_1d.tex <==
60.2

==> stats/againstv8_min_v8_baseline.tex <==
67

==> stats/againstv8_min_v8_baseline_1d.tex <==
67.1

==> stats/againstv8_min_v8_full.tex <==
10

==> stats/againstv8_min_v8_full_1d.tex <==
10.0

==> stats/againstv8_min_v8_no_inlining.tex <==
24

==> stats/againstv8_min_v8_no_inlining_1d.tex <==
23.6

==> stats/againstv8_num_above_v8_baseline.tex <==
25

==> stats/againstv8_num_above_v8_baseline_1d.tex <==
25.0

==> stats/againstv8_num_above_v8_full.tex <==
3

==> stats/againstv8_num_above_v8_full_1d.tex <==
3.0

==> stats/againstv8_num_above_v8_no_inlining.tex <==
5

==> stats/againstv8_num_above_v8_no_inlining_1d.tex <==
5.0

==> stats/againstv8_num_below_v8_baseline.tex <==
1

==> stats/againstv8_num_below_v8_baseline_1d.tex <==
1.0

==> stats/againstv8_num_below_v8_full.tex <==
23

==> stats/againstv8_num_below_v8_full_1d.tex <==
23.0

==> stats/againstv8_num_below_v8_no_inlining.tex <==
21

==> stats/againstv8_num_below_v8_no_inlining_1d.tex <==
21.0

==> stats/callknown_decr_entry+cont_spec.tex <==
3

==> stats/callknown_decr_entry+cont_spec_1d.tex <==
2.5

==> stats/callknown_decr_entry_spec.tex <==
3

==> stats/callknown_decr_entry_spec_1d.tex <==
2.6

==> stats/callknown_decr_typed_shapes.tex <==
10

==> stats/callknown_decr_typed_shapes_1d.tex <==
10.4

==> stats/callknown_incr_entry+cont_spec.tex <==
-3

==> stats/callknown_incr_entry+cont_spec_1d.tex <==
-2.5

==> stats/callknown_incr_entry_spec.tex <==
-3

==> stats/callknown_incr_entry_spec_1d.tex <==
-2.6

==> stats/callknown_incr_typed_shapes.tex <==
-10

==> stats/callknown_incr_typed_shapes_1d.tex <==
-10.4

==> stats/callknown_max_decr_entry+cont_spec.tex <==
29

==> stats/callknown_max_decr_entry+cont_spec_1d.tex <==
29.1

==> stats/callknown_max_decr_entry_spec.tex <==
29

==> stats/callknown_max_decr_entry_spec_1d.tex <==
29.1

==> stats/callknown_max_decr_typed_shapes.tex <==
100

==> stats/callknown_max_decr_typed_shapes_1d.tex <==
99.9

==> stats/callknown_max_entry+cont_spec.tex <==
100

==> stats/callknown_max_entry+cont_spec_1d.tex <==
100.0

==> stats/callknown_max_entry_spec.tex <==
100

==> stats/callknown_max_entry_spec_1d.tex <==
100.0

==> stats/callknown_max_incr_entry+cont_spec.tex <==
0

==> stats/callknown_max_incr_entry+cont_spec_1d.tex <==
0.0

==> stats/callknown_max_incr_entry_spec.tex <==
0

==> stats/callknown_max_incr_entry_spec_1d.tex <==
0.0

==> stats/callknown_max_incr_typed_shapes.tex <==
0

==> stats/callknown_max_incr_typed_shapes_1d.tex <==
0.0

==> stats/callknown_max_typed_shapes.tex <==
100

==> stats/callknown_max_typed_shapes_1d.tex <==
100.0

==> stats/callknown_mean_entry+cont_spec_1d.tex <==
97.5

==> stats/callknown_mean_entry_spec.tex <==
97

==> stats/callknown_mean_entry_spec_1d.tex <==
97.4

==> stats/callknown_mean_typed_shapes.tex <==
90

==> stats/callknown_mean_typed_shapes_1d.tex <==
89.6

==> stats/callknown_min_entry+cont_spec.tex <==
71

==> stats/callknown_min_entry+cont_spec_1d.tex <==
70.9

==> stats/callknown_min_entry_spec.tex <==
71

==> stats/callknown_min_entry_spec_1d.tex <==
70.9

==> stats/callknown_min_typed_shapes.tex <==
0

==> stats/callknown_min_typed_shapes_1d.tex <==
0.1

==> stats/callknown_num_above_entry+cont_spec.tex <==
0

==> stats/callknown_num_above_entry+cont_spec_1d.tex <==
0.0

==> stats/callknown_num_above_entry_spec.tex <==
0

==> stats/callknown_num_above_entry_spec_1d.tex <==
0.0

==> stats/callknown_num_above_typed_shapes.tex <==
0

==> stats/callknown_num_above_typed_shapes_1d.tex <==
0.0

==> stats/callknown_num_below_entry+cont_spec.tex <==
8

==> stats/callknown_num_below_entry+cont_spec_1d.tex <==
8.0

==> stats/callknown_num_below_entry_spec.tex <==
9

==> stats/callknown_num_below_entry_spec_1d.tex <==
9.0

==> stats/callknown_num_below_typed_shapes.tex <==
12

==> stats/callknown_num_below_typed_shapes_1d.tex <==
12.0

==> stats/codesize_decr_entry+cont_spec.tex <==
-2

==> stats/codesize_decr_entry+cont_spec_1d.tex <==
-2.2

==> stats/codesize_decr_entry_spec.tex <==
-2

==> stats/codesize_decr_entry_spec_1d.tex <==
-2.4

==> stats/codesize_incr_entry+cont_spec.tex <==
2

==> stats/codesize_incr_entry_spec.tex <==
2

==> stats/codesize_incr_entry_spec_1d.tex <==
2.4

==> stats/codesize_max_decr_entry+cont_spec.tex <==
9

==> stats/codesize_max_decr_entry+cont_spec_1d.tex <==
8.8

==> stats/codesize_max_decr_entry_spec.tex <==
1

==> stats/codesize_max_decr_entry_spec_1d.tex <==
0.9

==> stats/codesize_max_entry+cont_spec.tex <==
108

==> stats/codesize_max_entry+cont_spec_1d.tex <==
107.6

==> stats/codesize_max_entry_spec.tex <==
107

==> stats/codesize_max_entry_spec_1d.tex <==
106.6

==> stats/codesize_max_incr_entry+cont_spec.tex <==
8

==> stats/codesize_max_incr_entry_spec.tex <==
7

==> stats/codesize_max_incr_entry_spec_1d.tex <==
6.6

==> stats/codesize_mean_entry+cont_spec.tex <==
102

==> stats/codesize_mean_entry+cont_spec_1d.tex <==
102.2

==> stats/codesize_mean_entry_spec.tex <==
102

==> stats/codesize_mean_entry_spec_1d.tex <==
102.4

==> stats/codesize_min_entry+cont_spec.tex <==
91

==> stats/codesize_min_entry+cont_spec_1d.tex <==
91.2

==> stats/codesize_min_entry_spec.tex <==
99

==> stats/codesize_min_entry_spec_1d.tex <==
99.1

==> stats/codesize_num_above_entry+cont_spec.tex <==
23

==> stats/codesize_num_above_entry+cont_spec_1d.tex <==
23.0

==> stats/codesize_num_above_entry_spec.tex <==
25

==> stats/codesize_num_above_entry_spec_1d.tex <==
25.0

==> stats/codesize_num_below_entry+cont_spec.tex <==
3

==> stats/codesize_num_below_entry+cont_spec_1d.tex <==
3.0

==> stats/codesize_num_below_entry_spec.tex <==
1

==> stats/codesize_num_below_entry_spec_1d.tex <==
1.0

==> stats/comptime_decr_entry+cont_spec.tex <==
-1

==> stats/comptime_decr_entry+cont_spec_1d.tex <==
-1.0

==> stats/comptime_decr_entry_spec.tex <==
-1

==> stats/comptime_decr_entry_spec_1d.tex <==
-1.0

==> stats/comptime_incr_entry+cont_spec.tex <==
1

==> stats/comptime_incr_entry_spec.tex <==
1

==> stats/comptime_incr_entry_spec_1d.tex <==
1.0

==> stats/comptime_max_decr_entry+cont_spec.tex <==
3

==> stats/comptime_max_decr_entry+cont_spec_1d.tex <==
2.9

==> stats/comptime_max_decr_entry_spec.tex <==
-0

==> stats/comptime_max_decr_entry_spec_1d.tex <==
-0.2

==> stats/comptime_max_entry+cont_spec.tex <==
105

==> stats/comptime_max_entry+cont_spec_1d.tex <==
104.7

==> stats/comptime_max_entry_spec.tex <==
105

==> stats/comptime_max_entry_spec_1d.tex <==
104.7

==> stats/comptime_max_incr_entry+cont_spec.tex <==
5

==> stats/comptime_max_incr_entry_spec.tex <==
5

==> stats/comptime_max_incr_entry_spec_1d.tex <==
4.7

==> stats/comptime_mean_entry+cont_spec.tex <==
101

==> stats/comptime_mean_entry+cont_spec_1d.tex <==
101.0

==> stats/comptime_mean_entry_spec.tex <==
101

==> stats/comptime_mean_entry_spec_1d.tex <==
101.0

==> stats/comptime_min_entry+cont_spec.tex <==
97

==> stats/comptime_min_entry+cont_spec_1d.tex <==
97.1

==> stats/comptime_min_entry_spec.tex <==
100

==> stats/comptime_min_entry_spec_1d.tex <==
100.2

==> stats/comptime_num_above_entry+cont_spec.tex <==
23

==> stats/comptime_num_above_entry+cont_spec_1d.tex <==
23.0

==> stats/comptime_num_above_entry_spec.tex <==
26

==> stats/comptime_num_above_entry_spec_1d.tex <==
26.0

==> stats/comptime_num_below_entry+cont_spec.tex <==
3

==> stats/comptime_num_below_entry+cont_spec_1d.tex <==
3.0

==> stats/comptime_num_below_entry_spec.tex <==
0

==> stats/comptime_num_below_entry_spec_1d.tex <==
0.0

==> stats/exectime_decr_entry+cont_spec.tex <==
14

==> stats/exectime_decr_entry_spec.tex <==
12

==> stats/exectime_decr_entry_spec_1d.tex <==
12.3

==> stats/exectime_incr_entry+cont_spec.tex <==
-14

==> stats/exectime_incr_entry+cont_spec_1d.tex <==
-14.5

==> stats/exectime_incr_entry_spec.tex <==
-12

==> stats/exectime_incr_entry_spec_1d.tex <==
-12.3

==> stats/exectime_max_decr_entry+cont_spec_1d.tex <==
55.6

==> stats/exectime_max_decr_entry_spec.tex <==
56

==> stats/exectime_max_decr_entry_spec_1d.tex <==
55.6

==> stats/exectime_max_entry+cont_spec.tex <==
101

==> stats/exectime_max_entry+cont_spec_1d.tex <==
101.3

==> stats/exectime_max_entry_spec.tex <==
102

==> stats/exectime_max_entry_spec_1d.tex <==
102.5

==> stats/exectime_max_incr_entry+cont_spec.tex <==
1

==> stats/exectime_max_incr_entry+cont_spec_1d.tex <==
1.3

==> stats/exectime_max_incr_entry_spec.tex <==
2

==> stats/exectime_max_incr_entry_spec_1d.tex <==
2.5

==> stats/exectime_mean_entry+cont_spec.tex <==
86

==> stats/exectime_mean_entry+cont_spec_1d.tex <==
85.5

==> stats/exectime_mean_entry_spec.tex <==
88

==> stats/exectime_mean_entry_spec_1d.tex <==
87.7

==> stats/exectime_min_entry+cont_spec.tex <==
44

==> stats/exectime_min_entry+cont_spec_1d.tex <==
44.4

==> stats/exectime_min_entry_spec.tex <==
44

==> stats/exectime_min_entry_spec_1d.tex <==
44.4

==> stats/exectime_num_above_entry+cont_spec.tex <==
3

==> stats/exectime_num_above_entry+cont_spec_1d.tex <==
3.0

==> stats/exectime_num_above_entry_spec.tex <==
3

==> stats/exectime_num_above_entry_spec_1d.tex <==
3.0

==> stats/exectime_num_below_entry+cont_spec.tex <==
23

==> stats/exectime_num_below_entry+cont_spec_1d.tex <==
23.0

==> stats/exectime_num_below_entry_spec.tex <==
23

==> stats/exectime_num_below_entry_spec_1d.tex <==
23.0

==> stats/invs_per_fun_mean_1d.tex <==
10.2

==> stats/num_benchs_1d.tex <==
26.0

==> stats/ret_tag_known_mean_1d.tex <==
81.0

==> stats/shapetests_decr_entry+cont_spec.tex <==
54

==> stats/shapetests_decr_entry+cont_spec_1d.tex <==
53.7

==> stats/shapetests_decr_entry_spec.tex <==
31

==> stats/shapetests_decr_entry_spec_1d.tex <==
30.5

==> stats/shapetests_decr_typed_shapes.tex <==
25

==> stats/shapetests_decr_typed_shapes_1d.tex <==
24.9

==> stats/shapetests_incr_entry+cont_spec.tex <==
-54

==> stats/shapetests_incr_entry+cont_spec_1d.tex <==
-53.7

==> stats/shapetests_incr_entry_spec.tex <==
-31

==> stats/shapetests_incr_entry_spec_1d.tex <==
-30.5

==> stats/shapetests_incr_typed_shapes.tex <==
-25

==> stats/shapetests_incr_typed_shapes_1d.tex <==
-24.9

==> stats/shapetests_max_decr_entry+cont_spec.tex <==
100

==> stats/shapetests_max_decr_entry+cont_spec_1d.tex <==
99.9

==> stats/shapetests_max_decr_entry_spec.tex <==
100

==> stats/shapetests_max_decr_entry_spec_1d.tex <==
99.9

==> stats/shapetests_max_decr_typed_shapes.tex <==
100

==> stats/shapetests_max_decr_typed_shapes_1d.tex <==
99.9

==> stats/shapetests_max_entry+cont_spec.tex <==
126

==> stats/shapetests_max_entry+cont_spec_1d.tex <==
125.7

==> stats/shapetests_max_entry_spec.tex <==
131

==> stats/shapetests_max_entry_spec_1d.tex <==
131.5

==> stats/shapetests_max_incr_entry+cont_spec.tex <==
26

==> stats/shapetests_max_incr_entry+cont_spec_1d.tex <==
25.7

==> stats/shapetests_max_incr_entry_spec.tex <==
31

==> stats/shapetests_max_incr_entry_spec_1d.tex <==
31.5

==> stats/shapetests_max_incr_typed_shapes.tex <==
34

==> stats/shapetests_max_incr_typed_shapes_1d.tex <==
34.4

==> stats/shapetests_max_typed_shapes.tex <==
134

==> stats/shapetests_max_typed_shapes_1d.tex <==
134.4

==> stats/shapetests_mean_entry+cont_spec.tex <==
46

==> stats/shapetests_mean_entry+cont_spec_1d.tex <==
46.3

==> stats/shapetests_mean_entry_spec.tex <==
69

==> stats/shapetests_mean_entry_spec_1d.tex <==
69.5

==> stats/shapetests_mean_typed_shapes.tex <==
75

==> stats/shapetests_mean_typed_shapes_1d.tex <==
75.1

==> stats/shapetests_min_entry+cont_spec.tex <==
0

==> stats/shapetests_min_entry+cont_spec_1d.tex <==
0.1

==> stats/shapetests_min_entry_spec.tex <==
0

==> stats/shapetests_min_entry_spec_1d.tex <==
0.1

==> stats/shapetests_min_typed_shapes.tex <==
0

==> stats/shapetests_min_typed_shapes_1d.tex <==
0.1

==> stats/shapetests_num_above_entry+cont_spec.tex <==
2

==> stats/shapetests_num_above_entry+cont_spec_1d.tex <==
2.0

==> stats/shapetests_num_above_entry_spec.tex <==
3

==> stats/shapetests_num_above_entry_spec_1d.tex <==
3.0

==> stats/shapetests_num_above_typed_shapes.tex <==
3

==> stats/shapetests_num_above_typed_shapes_1d.tex <==
3.0

==> stats/shapetests_num_below_entry+cont_spec.tex <==
24

==> stats/shapetests_num_below_entry+cont_spec_1d.tex <==
24.0

==> stats/shapetests_num_below_entry_spec.tex <==
23

==> stats/shapetests_num_below_entry_spec_1d.tex <==
23.0

==> stats/shapetests_num_below_typed_shapes.tex <==
23

==> stats/shapetests_num_below_typed_shapes_1d.tex <==
23.0

==> stats/testcounts_decr_analysis.tex <==
92

==> stats/testcounts_decr_entry+cont_spec.tex <==
94

==> stats/testcounts_decr_entry_spec_1d.tex <==
89.2

==> stats/testcounts_decr_intra_bbv_1d.tex <==
60.2

==> stats/testcounts_decr_typed_shapes_1d.tex <==
77.6

==> stats/testcounts_incr_analysis.tex <==
-92

==> stats/testcounts_incr_analysis_1d.tex <==
-91.7

==> stats/testcounts_incr_entry+cont_spec.tex <==
-94

==> stats/testcounts_incr_entry+cont_spec_1d.tex <==
-94.3

==> stats/testcounts_incr_entry_spec.tex <==
-89

==> stats/testcounts_incr_entry_spec_1d.tex <==
-89.2

==> stats/testcounts_incr_intra_bbv.tex <==
-60

==> stats/testcounts_incr_intra_bbv_1d.tex <==
-60.2

==> stats/testcounts_incr_typed_shapes.tex <==
-78

==> stats/testcounts_incr_typed_shapes_1d.tex <==
-77.6

==> stats/testcounts_max_analysis.tex <==
25

==> stats/testcounts_max_analysis_1d.tex <==
24.9

==> stats/testcounts_max_decr_analysis.tex <==
100

==> stats/testcounts_max_decr_analysis_1d.tex <==
100.0

==> stats/testcounts_max_decr_entry+cont_spec.tex <==
100

==> stats/testcounts_max_decr_entry+cont_spec_1d.tex <==
100.0

==> stats/testcounts_max_decr_entry_spec.tex <==
100

==> stats/testcounts_max_decr_entry_spec_1d.tex <==
100.0

==> stats/testcounts_max_decr_intra_bbv.tex <==
96

==> stats/testcounts_max_decr_intra_bbv_1d.tex <==
96.3

==> stats/testcounts_max_decr_typed_shapes.tex <==
100

==> stats/testcounts_max_decr_typed_shapes_1d.tex <==
99.9

==> stats/testcounts_max_entry+cont_spec.tex <==
19

==> stats/testcounts_max_entry+cont_spec_1d.tex <==
19.3

==> stats/testcounts_max_entry_spec.tex <==
28

==> stats/testcounts_max_entry_spec_1d.tex <==
28.0

==> stats/testcounts_max_incr_analysis.tex <==
-75

==> stats/testcounts_max_incr_analysis_1d.tex <==
-75.1

==> stats/testcounts_max_incr_entry+cont_spec.tex <==
-81

==> stats/testcounts_max_incr_entry+cont_spec_1d.tex <==
-80.7

==> stats/testcounts_max_incr_entry_spec.tex <==
-72

==> stats/testcounts_max_incr_entry_spec_1d.tex <==
-72.0

==> stats/testcounts_max_incr_intra_bbv.tex <==
-0

==> stats/testcounts_max_incr_intra_bbv_1d.tex <==
-0.2

==> stats/testcounts_max_incr_typed_shapes.tex <==
-41

==> stats/testcounts_max_incr_typed_shapes_1d.tex <==
-41.2

==> stats/testcounts_max_intra_bbv.tex <==
100

==> stats/testcounts_max_intra_bbv_1d.tex <==
99.8

==> stats/testcounts_max_typed_shapes.tex <==
59

==> stats/testcounts_max_typed_shapes_1d.tex <==
58.8

==> stats/testcounts_mean_analysis.tex <==
8

==> stats/testcounts_mean_analysis_1d.tex <==
8.3

==> stats/testcounts_mean_entry+cont_spec.tex <==
6

==> stats/testcounts_mean_entry+cont_spec_1d.tex <==
5.7

==> stats/testcounts_mean_entry_spec.tex <==
11

==> stats/testcounts_mean_entry_spec_1d.tex <==
10.8

==> stats/testcounts_mean_intra_bbv.tex <==
40

==> stats/testcounts_mean_intra_bbv_1d.tex <==
39.8

==> stats/testcounts_mean_typed_shapes.tex <==
22

==> stats/testcounts_mean_typed_shapes_1d.tex <==
22.4

==> stats/testcounts_min_analysis.tex <==
0

==> stats/testcounts_min_analysis_1d.tex <==
0.0

==> stats/testcounts_min_entry+cont_spec.tex <==
0

==> stats/testcounts_min_entry+cont_spec_1d.tex <==
0.0

==> stats/testcounts_min_entry_spec.tex <==
0

==> stats/testcounts_min_entry_spec_1d.tex <==
0.0

==> stats/testcounts_min_intra_bbv.tex <==
4

==> stats/testcounts_min_intra_bbv_1d.tex <==
3.7

==> stats/testcounts_min_typed_shapes.tex <==
0

==> stats/testcounts_min_typed_shapes_1d.tex <==
0.1

==> stats/testcounts_num_above_analysis.tex <==
0

==> stats/testcounts_num_above_analysis_1d.tex <==
0.0

==> stats/testcounts_num_above_entry+cont_spec.tex <==
0

==> stats/testcounts_num_above_entry+cont_spec_1d.tex <==
0.0

==> stats/testcounts_num_above_entry_spec.tex <==
0

==> stats/testcounts_num_above_entry_spec_1d.tex <==
0.0

==> stats/testcounts_num_above_intra_bbv.tex <==
0

==> stats/testcounts_num_above_intra_bbv_1d.tex <==
0.0

==> stats/testcounts_num_above_typed_shapes.tex <==
0

==> stats/testcounts_num_above_typed_shapes_1d.tex <==
0.0

==> stats/testcounts_num_below_analysis.tex <==
26

==> stats/testcounts_num_below_analysis_1d.tex <==
26.0

==> stats/testcounts_num_below_entry+cont_spec.tex <==
26

==> stats/testcounts_num_below_entry+cont_spec_1d.tex <==
26.0

==> stats/testcounts_num_below_entry_spec.tex <==
26

==> stats/testcounts_num_below_entry_spec_1d.tex <==
26.0

==> stats/testcounts_num_below_intra_bbv.tex <==
26

==> stats/testcounts_num_below_intra_bbv_1d.tex <==
26.0

==> stats/testcounts_num_below_typed_shapes.tex <==
26

==> stats/testcounts_num_below_typed_shapes_1d.tex <==
26.0
